Hierarchical Performance Modeling for Ranking Dense Linear Algebra Algorithms

A large class of dense linear algebra operations, such as LU decomposition or inversion of a triangular matrix, are usually performed by blocked algorithms. For one such operation, typically, not only one but many algorithmic variants exist; depending on computing architecture, libraries and problem size, each variant attains a different performances. We propose methods and tools to rank the algorithmic variants according to their performance for a given scenario without executing them. For this purpose, we identify the routines upon which the algorithms are built. A first tool - the Sampler - measures the performance of these routines. Using the Sampler, a second tool models their performance. The generated models are then used to predict the performance of the considered algorithms. For a given scenario, these predictions allow us to correctly rank the algorithms according to their performance without executing them. With the help of the same tools, algorithmic parameters such as block-size can be optimally tuned.

==> Makefile <==
PDFLATEX = pdflatex -shell-escape

TARGET = main.pdf

TEXFILES = *.tex figures/*.tex

default: twice

once: 
	time $(PDFLATEX) main

twice:
	make once
	make once

figs:
	time make -j 4 -B -f main.makefile

bib:
	bibtex main

all:
	make once
	make figs
	make bib
	make once
	make figs
	make once

bg:
	make once < /dev/null 2>&1 1> /dev/null &

figtest:
	$(PDFLATEX) figtest
	#time make -j 2 -B -f figtest.makefile
	#$(PDFLATEX) figtest.tex

title:
	$(PDFLATEX) title

check: $(TEXFILES)
	for file in $(TEXFILES); \
	do \
		aspell --lang=EN --mode=tex check $$file; \
	done

clean:
	rm -rf main.{aux,log,toc,pdf,lof,out,figlist,makefile,pyg}


==> figures/modeling.res.ticks.me.tex <==
\begin{figure}[t]
% %    \tikzset{external/export=true}
    \newcommand{\regionsplot}[1]{
        \begin{tikzpicture}
            \begin{axis}[
                twocolplot,
                axis equal image=true,
                xlabel={\texttt m},
                ylabel={\texttt n},
                xtick={0,256,...,1024},
                ytick={0,256,...,1024},
                xmax=1024,
                ymax=1024
            ]
                \coordinate (oi) at (axis description cs: 0, 1);
                \coordinate (io) at (axis description cs: 1, 0);
            \end{axis}

            \foreach \ax/\ay/\bx/\by/\e in {#1} {
                \pgfmathparse{100 * max(0, min(1, 1 * (1 - 5*\e)))}
                \filldraw[fill=plot2!\pgfmathresult!plot1, opacity=.9] ($\ax/1024*(io) + \ay/1024*(oi)$) rectangle ($\bx/1024*(io) + \by/1024*(oi)$);
            }
        \end{tikzpicture}
    }
    \centering
    \subfloat[error bound = 10\%, expansion direction = $\nearrow$, initial width = 128]{
        \label{fig:modeling.res.ticks.me:a10.sg32.dr}
        \regionsplot{
            %figures/data/modeling.res.ticks.me/a10.sg32.dr.dat
            8/8/104/104/1.00469552302,
            112/8/224/504/0.0925378117453,
            8/112/104/208/0.0899962466816,
            8/216/104/312/0.136738988956,
            8/320/104/416/0.205671004464,
            8/424/104/520/0.337808607959,
            232/8/424/248/0.0895894822351,
            112/512/216/944/0.0888837091473,
            8/528/104/624/0.11464252529,
            8/632/104/1008/0.0832475826006,
            432/8/528/104/0.341494934763,
            232/256/368/352/0.0985248840035,
            112/952/208/1024/0.151603768446,
            224/512/320/608/0.120270481454,
            8/1016/136/1024/0.088493281342,
            536/8/824/120/0.0990907381512,
            432/112/704/344/0.0981517499468,
            216/952/312/1024/0.124083089475,
            224/616/704/848/0.0969178070244,
            328/512/1000/1016/0.0967287902334,
            232/360/328/456/0.124388784778,
            376/256/1024/392/0.092724544515,
            336/360/1016/1008/0.0958524737678,
            232/464/328/560/0.129467784303,
            712/128/1024/1024/0.0869214186458,
            832/8/928/104/0.105363710864,
            832/112/1024/1024/0.0552884313051,
            936/8/1024/624/0.0994502179859,
            224/856/448/1008/0.0953467774158,
            320/1016/800/1024/0.0750460199508
        }
    }
    \vfill
    \subfloat[error bound = 10\%, expansion direction = $\swarrow$, initial width = 128]{
        \label{fig:modeling.res.ticks.me:a10.sg32.dl}
        \regionsplot{
            %figures/data/modeling.res.ticks.me/a10.sg32.dl.dat
            %32580 samples
            %.0699 avg acc
            144/408/1024/1024/0.064230745417,
            536/8/1024/400/0.0614626491845,
            40/928/136/1024/0.176948662506,
            32/192/136/920/0.0749014556158,
            8/928/32/1024/0.0462208519538,
            168/168/528/400/0.0884647795771,
            8/824/24/920/0.106224004915,
            8/720/24/816/0.108707652278,
            8/616/24/712/0.143674342052,
            160/48/528/160/0.0943284348788,
            64/64/160/400/0.0511439972596,
            8/512/24/608/0.137464637655,
            8/272/24/504/0.0945303973329,
            8/88/56/184/0.127791203696,
            56/8/152/56/0.0829470155189,
            8/8/56/80/0.0571283006961,
            184/8/528/40/0.0678138682488,
            8/168/24/264/0.200775124444,
            80/8/176/40/0.104301590893
        }
    }

    \subfloat[error bound = 5\%, expansion direction = $\swarrow$, initial width = 128]{
        \label{fig:modeling.res.ticks.me:a5.sg32.dl}
        \regionsplot{
            %figures/data/modeling.res.ticks.me/a5.sg32.dl.dat
            %53550 samples
            %.0580 avg acc
            512/192/1024/1024/0.0482120288048,
            152/552/504/1024/0.0439441743443,
            744/8/1024/184/0.045209148553,
            368/48/736/184/0.0457191034119,
            224/88/504/544/0.0498135669515,
            48/928/144/1024/0.146546362558,
            8/928/40/1024/0.0366798615078,
            48/824/144/920/0.17609281073,
            48/720/144/816/0.113799537273,
            8/720/40/816/0.0575027405058,
            24/304/144/712/0.0464559420081,
            640/8/736/40/0.0517294670242,
            8/824/40/920/0.164491358635,
            528/8/632/40/0.0298791729969,
            56/216/216/544/0.0427817539938,
            144/8/360/80/0.0471980240611,
            8/616/16/712/0.128335814423,
            424/8/520/40/0.850090470963,
            8/512/16/608/0.129485329486,
            40/8/136/80/0.126668878985,
            320/8/416/40/0.163671309602,
            8/408/16/504/0.0994956515629,
            8/304/16/400/0.108574361292,
            8/200/48/296/0.143784132967,
            56/112/216/208/0.0433732976348,
            8/96/48/192/0.194636783622,
            120/8/216/104/0.0870420981146,
            8/8/48/88/0.478092293419,
            16/8/112/104/0.470426091606
        }
    }
    \vfill
    \subfloat[error bound = 5\%, expansion direction = $\swarrow$, initial width = 64]{
        \label{fig:modeling.res.ticks.me:a5.sg16.dl}
        \regionsplot{
            %figures/data/modeling.res.ticks.me/a5.sg16.dl.dat
            %138290 samples
            %.0597 avg acc
            472/176/1024/1024/0.0469040916926,
            416/976/464/1024/0.0532795630622,
            720/8/1024/168/0.0470819522827,
            232/880/408/1024/0.0497572243788,
            288/656/464/968/0.0498514160808,
            536/48/712/168/0.0443373474728,
            176/976/224/1024/0.065508044443,
            120/976/168/1024/0.153568721594,
            176/888/224/968/0.0451571203487,
            232/824/280/872/0.0448652020619,
            256/592/464/648/0.0482581518478,
            64/976/112/1024/0.19073780162,
            8/976/56/1024/0.030969136151,
            664/8/712/40/0.0636646129475,
            480/120/528/168/0.0654420816894,
            120/920/168/968/0.135854507789,
            176/832/224/880/0.0676723878788,
            528/8/656/40/0.0346553619416,
            480/64/528/112/0.1197166747,
            424/120/472/168/0.0887150917635,
            176/776/224/824/0.0704173023976,
            120/824/168/872/0.182387707018,
            232/688/280/816/0.0474240593529,
            8/920/56/968/0.0841096128778,
            120/864/168/912/0.137462167925,
            64/920/112/968/0.185772047315,
            424/64/472/112/0.0965392941138,
            480/8/528/56/0.367512858912,
            368/120/416/168/0.101162750184,
            328/536/464/584/0.0498703150081,
            64/776/112/824/0.115998379257,
            64/824/112/872/0.143706965844,
            8/864/56/912/0.130987223145,
            64/864/112/912/0.154085349155,
            424/8/472/56/0.304757246881,
            8/776/56/824/0.0641376888399,
            64/720/112/768/0.0712288951234,
            8/808/56/856/0.230965541805,
            368/8/416/56/0.134330569443,
            8/720/56/768/0.10112949836,
            64/664/112/712/0.0538589130631,
            312/8/360/56/0.121931171322,
            8/664/56/712/0.156454833983,
            64/608/112/656/0.0705459585713,
            248/8/304/56/0.0400464335912,
            8/608/56/656/0.0643646899951,
            40/168/112/600/0.0410735636557,
            120/768/168/816/0.137948959692,
            176/720/224/768/0.0931684574737,
            232/632/280/680/0.0644471485231,
            416/480/464/528/0.0521212790588,
            272/536/320/584/0.0850841148138,
            120/712/168/760/0.163786022049,
            176/664/224/712/0.0864073377341,
            232/480/280/528/0.0661705198597,
            200/576/248/624/0.0458205996204,
            216/536/264/584/0.0840573987667,
            360/480/408/528/0.0478712933274,
            280/176/464/472/0.0428624697569,
            104/656/168/704/0.0128350463565,
            176/608/224/656/0.114285333573,
            192/8/240/56/0.0567630475192,
            8/552/32/600/0.14955288781,
            64/112/112/160/0.0513714476488,
            304/416/352/528/0.0451269835135,
            120/576/168/624/0.160086525026,
            144/552/192/600/0.139674626966,
            160/520/208/568/0.106307490237,
            120/600/168/648/0.149455854243,
            88/520/136/568/0.102469845805,
            8/496/32/544/0.128770882757,
            104/496/152/544/0.0838182418266,
            120/464/168/512/0.111771677753,
            8/112/56/160/0.0763583825661,
            56/8/112/104/0.037526133229,
            144/464/192/512/0.163603094003,
            160/464/208/512/0.162289374408,
            368/64/416/112/0.120067151782,
            136/8/184/56/0.0488337557606,
            312/120/360/168/0.133510920059,
            224/424/272/472/0.116687089085,
            8/440/32/488/0.127346382278,
            176/32/360/112/0.0428413754193,
            256/120/304/168/0.113527610467,
            224/368/272/416/0.108301386057,
            168/424/216/472/0.158876071371,
            224/312/272/360/0.125560501131,
            248/480/296/528/0.0588965805361,
            168/360/216/408/0.115684613096,
            200/8/248/168/0.047411023609,
            56/176/160/360/0.0417173775091,
            168/56/216/352/0.0455897036574,
            224/256/272/304/0.0984174766414,
            168/368/216/416/0.1242892291,
            176/480/224/528/0.110404288417,
            112/144/160/456/0.0458260637867,
            8/384/32/432/0.1010340302,
            224/200/272/248/0.0813359915597,
            224/144/272/192/0.111661921397,
            80/8/128/24/0.0389232293718,
            8/312/32/360/0.152206169895,
            8/56/48/104/0.0682498281356,
            80/8/128/48/0.0889719448527,
            8/8/48/48/0.194705559387,
            112/88/160/136/0.0554784620143,
            8/328/32/376/0.141131602765,
            112/32/160/80/0.0518663101012,
            8/256/32/304/0.0908893775485,
            8/200/32/248/0.123700153613,
            8/144/32/192/0.140849060573
        }
    }

    \vspace{.5cm}
    \tikzset{external/export=false}

    \begin{tikzpicture}
        \coordinate (pos) at (0, 0);
        \filldraw[fill=plot1] (pos) +(-2.5, 0) rectangle +(2.5, -.5);
        \filldraw[path fading=west, fill=plot2] (pos) +(-2.5, 0) rectangle +(2.5, -.5);
        \path (pos) ++(-2.5, -.25) node[anchor=east] {error:};
        \path (pos) ++(2.5, -.25) node[anchor=west] {\phantom{error:}};
        \path (pos) ++(-2.5, -.5) node[anchor=north] {0.2};
        \path (pos) ++(2.5, -.5) node[anchor=north] {0};
        \draw[dashed] (pos) ++(-2.5, 0) ++($.5*(5, 0)$) -- ++(0, -.5) node[anchor=north] {0.1};
        \draw[dashed] (pos) ++(-2.5, 0) ++($.75*(5, 0)$) -- ++(0, -.5) node[anchor=north] {0.05};
    \end{tikzpicture}

    \caption{\metric{ticks} model for \texttt{dtrsm} with Model Expansion.}
    \label{fig:modeling.res.ticks.me}
\end{figure}

